Streaming Bayes GFlowNets

Bayes' rule naturally allows for inference refinement in a streaming fashion, without the need to recompute posteriors from scratch whenever new data arrives. In principle, Bayesian streaming is straightforward: we update our prior with the available data and use the resulting posterior as a prior when processing the next data chunk. In practice, however, this recipe entails i) approximating an intractable posterior at each time step; and ii) encapsulating results appropriately to allow for posterior propagation. For continuous state spaces, variational inference (VI) is particularly convenient due to its scalability and the tractability of variational posteriors. For discrete state spaces, however, state-of-the-art VI results in analytically intractable approximations that are ill-suited for streaming settings. To enable streaming Bayesian inference over discrete parameter spaces, we propose streaming Bayes GFlowNets (abbreviated as SB-GFlowNets) by leveraging the recently proposed GFlowNets -- a powerful class of amortized samplers for discrete compositional objects. Notably, SB-GFlowNet approximates the initial posterior using a standard GFlowNet and subsequently updates it using a tailored procedure that requires only the newly observed data. Our case studies in linear preference learning and phylogenetic inference showcase the effectiveness of SB-GFlowNets in sampling from an unnormalized posterior in a streaming setting. As expected, we also observe that SB-GFlowNets is significantly faster than repeatedly training a GFlowNet from scratch to sample from the full posterior.

==> drafts/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> early_draft.tex <==
\subsection{Uniform distributions and uniform flows}
\begin{itemize}
    \item A uniform flow of degree $g$ and height $h$ is a Markovian flow that models a uniform distribution, meaning all the leaf nodes have the same value. The policy of such flow consists in a function that takes the incoming flow and splits it equally between each of the g outgoing nodes.
\end{itemize}

To start let us consider the example of a flow trained on a uniform distribution and policy that takes the incoming flow and split it equally to all outgoing states. The resulting uniform distribution on the terminal nodes density is  represented by $\pi^*(x)=\frac{1}{g^h}$, for each terminal object in the domain $x \in \mathcal{X}$ and $|\mathcal{X}|=g^h$.

Let us consider the case that the policy at the root of the network introduces an error in the flow of size $\delta$, meaning that one children node now will receive a flow $\frac{F}{g}+\delta$ and the other $g-1$ will continue with $\frac{F}{g}$, which is equivalent to the policy with a probability density (after normalizing) that assigns a probability $\frac{F+g\delta}{g(F+\delta)}$ to one branch and $\frac{F}{g(F+\delta)}$ to the other $g-1$ branches. The total variation distance between this new density and the original policy (uniform probability for each $g$ branches) is $\epsilon(\delta, g)=(1-\frac{1}{g})\frac{\delta}{F+\delta}$. Now we denote the resulting sampling distribution induced by this modified flow as $\pi(x)$.


\begin{figure}[h]
    \center 
% https://q.uiver.app/#q=WzAsMTMsWzMsMCwiRitcXGRlbHRhIl0sWzIsMSwiXFxmcmFje0Z9e2d9K1xcZGVsdGEiXSxbNCwxLCJcXGZyYWN7Rn17Z31cXHRleHR7IH1cXHRyaWFuZ2xlIl0sWzIsMiwiXFx0cmlhbmdsZSJdLFswLDMsIlxcZnJhY3tGfXtnXmh9K1xcZGVsdGFfMSJdLFsxLDIsIlxcdHJpYW5nbGUiXSxbNSwyLCJcXHRyaWFuZ2xlIl0sWzQsMiwiXFx0cmlhbmdsZSJdLFsxLDMsIlxcZnJhY3tGfXtnXmh9K1xcZGVsdGFfMlxcdGV4dHsgIH1cXGxkb3RzICJdLFsyLDMsIlxcZnJhY3tGfXtnXmh9K1xcZGVsdGFfe2dee2gtMX19Il0sWzQsMywiXFxmcmFje0Z9e2deaH0iXSxbNSwzLCJcXGZyYWN7Rn17Z15ofSJdLFs2LDMsIlxcZnJhY3tGfXtnXmh9Il0sWzAsMSwiXFx0ZXh0e2RlZ3JlZSBnfSJdLFswLDJdLFsyLDZdLFsyLDddLFsxLDNdLFsxLDVdLFs1LDRdLFs1LDhdLFszLDldLFs3LDEwXSxbNiwxMV0sWzYsMTJdXQ==
\[\begin{tikzcd}
	&&& {F+\delta} \\
	&& {\frac{F}{g}+\delta} && {\frac{F}{g}\text{ }\triangle} \\
	& \triangle & \triangle && \triangle & \triangle \\
	{\frac{F}{g^h}+\delta_1} & {\frac{F}{g^h}+\delta_2\text{  }\ldots } & {\frac{F}{g^h}+\delta_{g^{h-1}}} && {\frac{F}{g^h}} & {\frac{F}{g^h}} & {\frac{F}{g^h}}
	\arrow["{\text{degree g}}", from=1-4, to=2-3]
	\arrow[from=1-4, to=2-5]
	\arrow[from=2-5, to=3-6]
	\arrow[from=2-5, to=3-5]
	\arrow[from=2-3, to=3-3]
	\arrow[from=2-3, to=3-2]
	\arrow[from=3-2, to=4-1]
	\arrow[from=3-2, to=4-2]
	\arrow[from=3-3, to=4-3]
	\arrow[from=3-5, to=4-5]
	\arrow[from=3-6, to=4-6]
	\arrow[from=3-6, to=4-7]
\end{tikzcd}\]
\caption{A flow network with a extra flow of $\delta$ in one of the branches of the initial state} 
    \label{fig:tree_graph} 
\end{figure}

Let $\mu$ and $\nu$ be two probability measures, then we denote $||\mu - \nu||_{\scaleto{\textbf{TV}}{3pt}}$ as the total variation distance between them. 

\begin{assumption}\label{as: gf_tree_unif}
 Let the pair $(G_T, F)$ be a flow network such that $G_T$ is a regular tree with degree $g$ and depth $h$. Furthermore, assume that $F$ spreads uniformly in the edges of $G_T$, then the target distribution $\pi^*$ generated by $(G_T, F)$ is uniform.      
\end{assumption}

\begin{theorem}[Total variation of the sampling distribution] Let $\delta >0$ and $\sum_{i=1}^{g^{h-1}} \delta_i = \delta$, where $\delta_i \in [0, \delta]$ for all $i \in \{1,2, \dots, g^{h-1}\}$. Suppose that we have the flow network $(G_T, F+\delta)$  abiding by Assumption~\ref{as: gf_tree_unif} besides the first edge from the root to a son where it has a $\delta$ increasing generating a new target distribution $\pi$. Then under these conditions describe the total variation distance between $\pi$ and $\pi^*$ is bounded above and below by the following
\begin{align*}
& \epsilon(\delta, g) \leq ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} \leq \epsilon(\delta, g^h) \quad \text{where}
\\
& \epsilon(a,b) := \Big(1 - \frac{1}{b} \Big) \frac{a}{F+a}\,.
\end{align*}
\end{theorem}

\begin{proof}
The terminal states of the modified flow network will have two types of nodes, with flow $\frac{F}{g^h}$ and $\frac{F}{g^h}+\delta_{i}$, with $\delta_i \geq 0$ and $\sum_{i=1}^{g^{h-1}} \delta_i = \delta$. We normalize those probabilities to obtain the individual probabilities for each terminal state, which determines the density of each sample. From that, we can proceed to compute the total variation distance between $\pi$ and $\pi^*$.
\begin{align*}
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &= \frac{1}{2}\sum_{x \in \mathcal{X}} | \pi(x)- \pi^*(x) | \\
                          &= \frac{1}{2}\left[(g^h-g^{h-1})\left|\frac{F}{g^h}\frac{1}{F+\delta} - \frac{1}{g^h}\right|+ \sum_{i=1}^{g^{h-1}} \left|\frac{F+g^h\delta_i}{g^h}\frac{1}{F+\delta} - \frac{1}{g^h}\right| \right] \\
                          &= \frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta+\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|}{g^h(F+\delta)}\right]
\end{align*}

We can lower bound $\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|$, by considering that $\sum_{i=1}^{g^{h-1}}(g^h\delta_i-\delta)=g^{h}\delta-g^{h-1}\delta$, taking the absolute value of the result and each element of the sum to obtain $g^{h}\delta-g^{h-1}\delta \leq \sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|$. Thus we obtain the lower bound 
\begin{align*}
\frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta+g^{h}\delta-g^{h-1}\delta}{g^h(F+\delta)}\right]&\leq \frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta+\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|}{g^h(F+\delta)}\right] \\
                       \left(1-\frac{1}{g}\right)\frac{\delta}{F+\delta} &\leq  ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} 
\end{align*}.

This lower bound is reached when all error terms in the terminal states have the same value $\delta_i = \frac{\delta}{g^h}$.

To upper bound $|g^h\delta_i-\delta|$ we apply the triangle inequality, obtaining $|g^h\delta_i-\delta| \leq g^h\delta_i+\delta$ and  $\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta| \leq g^h\delta+g^{h-1}\delta$, from which we obtain the upper bound
\begin{align*}
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq \frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta + g^{h}\delta+g^{h-1}\delta}{g^h(F+\delta)}\right] \\
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq \frac{\delta}{F+\delta}
\end{align*}.

To obtain a tighter bound we break the sum $\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|$ by partitioning the sum into the first $I$ terms $S_A=g^h\sum_{i=1}^{I}|\delta_i-\frac{\delta}{g^h}|$ with $\delta_i < \frac{\delta}{g^h}$ and subsequent $g^{h-1}-I$ terms $S_B=g^h\sum_{j=I+1}^{g^{h-1}}|\delta_j-\frac{\delta}{g^h}|$ with $\delta_j \geq \frac{\delta}{g^h}$. By construction, we know that $S_A+g^h\sum_{i=1}^{I}\delta_i+g^h\sum_{j=I+1}^{g^{h-1}}\delta_j-S_B=g^{h-1}\delta$, simplifying to $S_B-S_A=\delta(g^h-g^{h-1})$. We rewrite $S_A + S_B = S_B-S_A+2S_A=\delta(g^h-g^{h-1})+2S_A$, and by triangle inequality on $S_A$, we obtain the upper bound $\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|=S_A+S_B \leq g^h\delta-g^{h-1}\delta+2I\delta $. Setting $I=g^{h-1}-1$ (the biggest value it can have without breaking the constraints on $\delta_i$), it simplifies to $S_A+S_B \leq g^h\delta+g^{h-1}\delta-2\delta $

\begin{align*}
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq \frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta+\sum_{i=1}^{g^{h-1}}|g^h\delta_i-\delta|}{g^h(F+\delta)}\right] \\
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq \frac{1}{2}\left[\frac{g^h\delta-g^{h-1}\delta+g^h\delta+g^{h-1}\delta-2\delta }{g^h(F+\delta)}\right] \\
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq \left[\frac{g^h\delta-\delta }{g^h(F+\delta)}\right] \\
    ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} &\leq  \left(1-\frac{1}{g^h}\right)\frac{\delta}{F+\delta}
\end{align*}.
\end{proof}

\textcolor{red}{\begin{theorem}[Total variation of the sampling distribution] Let $\delta >0$ and $\sum_{i=1}^{n} \delta_i = \delta$, where $\delta_i \in [0, \delta]$. Suppose that we have the flow network $(G_n, F)$ which generates a target distribution $\pi^*$ uniform in the number of final vertices. Then if we increase the flow $F$ by $\delta$ in the same graph, that is $(G_n, F + \delta)$, generating a new target distribution $\pi$, the total variation distance between $\pi$ and $\pi^*$ is bounded above and below by the following
\begin{align*}
& ||\pi -\pi^*||_{\scaleto{\textbf{TV}}{3pt}} \leq \epsilon(\delta, n) \quad \text{where}
\\
& \epsilon(a,b) := \Big(1 - \frac{1}{b} \Big) \frac{a}{F+a}\,.
\end{align*}
\end{theorem}}




\section{Inherent limitations of policy networks}



\begin{figure}
    \center 
    \includegraphics[scale=.3]{gflownets_wl_test.pdf} 
    \caption{A state graph whose downstream distribution is not learnable by a GFlowNet with a policy network is
    parametrized by a 1-WL GNN.} 
    \label{fig:wl_graphs} 
\end{figure}

\begin{theorem}[Distributional constraints of GFlowNets] 
    Let $\mathcal{G} = \{(\mathbf{X}, \mathbf{A}) \colon \mathbf{A} \in \{0,
    1\}^{N \times N}\}$ be the set of equally featured graphs with adjacency matrix $\mathbf{A}$
    and features $\mathbf{r} \in \mathbb{R}^{d}$ ($\mathbf{X} = \mathbf{1}\mathbf{r}^{T} \in \mathbb{R}^{N \times d}$). Let $F_{\theta} \colon \mathcal{G} \rightarrow \Delta_{2}$ be the
    \textit{policy network} that maps a graph $G \in \mathcal{G}$ to a point within the simplex of action-probabilities $\Delta_{2} =
    \{(a^{(1)}, a^{(2)}) \colon a^{(1)} + a^{(2)} = 1 \text{ and
    } a^{(1)}, a^{(2)} \ge 0\}$. See Figure~\ref{fig:wl_graphs}. Suppose that the policy network is parametrized by an 1-WL GNN with parameters $\theta$. Let $\pi$ be a distribution on the
    graphs $\{G_{i} \colon i \in \{1, 2, 3, 4\}\}$ of Figure~\ref{fig:wl_graphs} with $\pi(G_{1}) = \pi(G_{2}) = \pi(G_{3}) =
    \frac{1}{6}$ and $\pi(G_{4}) = \frac{1}{2}$. In these settings, there does not exist a
    $\theta$ such that the downstream distribution induced by the policy network equals $\pi$. 
\end{theorem}

\begin{proof}
    Let $p_{\theta}(X | S_{o})$ be the marginal transition probability learned by the GFlowNet of reaching the state $X
    \in \mathcal{G}$
    through the generative process characterized by the state graph of Figure~\ref{fig:wl_graphs} and the policy network
    $F_{\theta}$. We will show that
    $p_{\theta}(G_{i} | S_{o})$ is -- for any $\theta$ -- necessarily different of $\pi(G_{i})$ for at least two graphs
    in $\pi$'s support. 

    For this, notice that the Markovity of the stochastic transitions learned by the GFlowNet
    entails that 
    $p_{\theta}(G_{1} | S_{o}) = p_{\theta}(N_{1} | S_{o}) p_{\theta}(G_{1} | N_{1})$, 
    $p_{\theta}(G_{2} | S_{o}) = p_{\theta}(N_{1} | S_{o}) p_{\theta}(G_{2} | N_{1})$, 
    $p_{\theta}(G_{3} | S_{o}) = p_{\theta}(N_{2} | S_{o}) p_{\theta}(G_{3} | N_{2})$ and  
    $p_{\theta}(G_{4} | S_{o}) = p_{\theta}(N_{2} | S_{o}) p_{\theta}(G_{4} | N_{2})$. 
    Notably, the indistinguishability of the graphs $N_{1}$ and $N_{2}$ according to the 1-WL 
    isomorphism test implies that $F_{\theta}(N_{1}) = F_{\theta}(N_{2})$ and hence the transition  
    probabilities must satisfy $p_{\theta}(G_{1} | N_{1}) = p_{\theta}(G_{3} | N_{2})$ and $p_{\theta}(G_{2} | N_{1}) =
    p_{\theta}(G_{4} | N_{2})$. 

    Contradictorily, suppose that there is a $\theta$ such that the policy network $F_{\theta}$ is perfectly adjusted to the target distribution $\pi$.
    Hence, $p_{\theta}(G_{i} | S_{o}) = \pi(G_{i})$ for each $i \in \{1, 2, 3, 4\}$. Nonetheless, the representational equivalence of
    $N_{1}$ and $N_{2}$ and the Markovian assumption imply that 

    \begin{equation*} 
        \begin{split} 
        p_{\theta}(N_{1} | S_{o}) = \frac{\pi(G_{1})}{p_{\theta} (G_{1} | N_{1})} 
        = \frac{\pi(G_{3})}{p_{\theta} (G_{3} | N_{2})} = p_{\theta}(N_{2} | S_{o}) 
        \text{ and that } \\ 
        p_{\theta}(N_{1} | S_{o}) = \frac{\pi(G_{2})}{p_{\theta}(G_{2} | N_{1})} \neq 
        \frac{\pi(G_{4})}{p_{\theta}(G_{4} | N_{2})} = p_{\theta}(N_{2} | S_{o}).
        % p_{\theta}(N_{1} | S_{o}) = 
    \end{split} 
    \end{equation*} 

   \noindent This contradiction guarantees that $p(G_{i} | S_{o})$ is necessarily different from $\pi(G_{i})$ for at
   least a pair of graphs and asseverates that the distribution characterized by the state graph of
   Figure~\ref{fig:wl_graphs} is unlearnable by a GFlowNet parametrized by a 1-WL GNN. 
\end{proof}

\begin{remark}
    The previous theorem states the limitations of a GFlowNet parametrized by a 1-WL GNN. The alternative use of a more
    expressive yet not permutationally invariant flow parametrization would entail a factorially large increase of the
    size of the state graph, as equivalent graphs with different labelling would be treated differently by the flow
    estimator, and lead to a computationally untractable problem. The next theorem characterizes a weak relationship
    between the size of the state graph and the statistical efficiency of a maximally entropic exploratory policy within the state graph.   
\end{remark}

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> section3_old.tex <==

We start our analysis by quantifying the consequences of a deviance from the flows' balance on the underlying marginal distribution over the terminal states. Our results highlight, on the one hand, that a lack of flow-balance upstream in the generative process is more damaging to the overall distributional accuracy of a GFlowNet than an equivalent imbalance nearer the terminal states; on the other hand, that a disruption of the detailed balance condition in a single edge may be catastrophically propagated within the network and severely damage the approximation to the target distribution. See the appendix for self-contained proofs of our results. 

\begin{figure}[t]
    \center 
    \def\spacing{-15pt}
\[\begin{tikzcd}
	&[\spacing]&[\spacing] {F+\delta} \\
	&[\spacing] {\frac{F}{g}+\delta} &[\spacing]&[\spacing]&[\spacing] {\frac{F}{g}} \\
% 	& \triangle & \triangle && \triangle & \triangle \\
    {\frac{F}{g^h}+\delta_1} &[\spacing] {\frac{F}{g^h}+\delta_2} &[\spacing]&[\spacing] % {\frac{F}{g^h}+\delta_{g^{h-1}}} 
    &[\spacing] {\frac{F}{g^h}} &[\spacing] {\frac{F}{g^h}} % & {\frac{F}{g^h}}
    \arrow["{\text{degree g}}", swap, from=1-3, to=2-2]
	\arrow[from=1-3, to=2-5]
	\arrow[from=2-5, to=3-6]
	\arrow[from=2-5, to=3-5]
	\arrow[from=2-2, to=3-1]
	\arrow[from=2-2, to=3-2] 
    % \arrow[from=3-2, to=4-1]
	% \arrow[from=3-2, to=4-2]
	% \arrow[from=3-3, to=4-3]
	% \arrow[from=3-5, to=4-5]
	% \arrow[from=3-6, to=4-6]
	% \arrow[from=3-6, to=4-7]
\end{tikzcd}\]
\caption{\textbf{Imbalanced flows in a regular tree} with width $g = 2$ and depth $h = 2$. The extra flow within the root's left child breaks the expected uniform distribution over the $g^{h}$ leaves.}
% \caption{\textbf{Imbalanced flow network in a tree.}}
% \caption{A flow network with a extra flow of $\delta$ in one of the branches of the initial state} 
    \label{fig:a} 
    % \label{fig:treesgraphs} 
\end{figure}

% \begin{theorem}[Total variation of the sampling distribution] Let $\delta >0$ and $\sum_{i=1}^{g^{h-1}} \delta_i = \delta$, where $\delta_i \in [0, \delta]$ for all $i \in \{1,2, \dots, g^{h-1}\}$. Suppose that we have the flow network $(G_T, F+\delta)$ abiding by Assumption~\ref{as: gf_tree_unif} besides the first edge from the root to a son where it has a $\delta$ increasing generating a new target distribution $\pi$ (see Figure [ref]).  Under these conditions, the total variation distance between $\pi$ and $\pi^*$ is bounded above and below by 
% \begin{align*}
% & \epsilon(\delta, g) \leq ||\pi - \pi^*||_{\scaleto{\textbf{TV}}{3pt}} \leq \epsilon(\delta, g^h) \quad \text{where}
% \\
% & \epsilon(a,b) := \Big(1 - \frac{1}{b} \Big) \frac{a}{F+a}\,.
% \end{align*}
% \end{theorem}


\vspace{4pt}\noindent\textbf{Bounds on TV for arbitrary state graphs.} We show that the intuition built upon the previous discussion relatively to tree-structured state graphs carries out to general acyclic generative processes, namely, (i) that an imbalanced edge reaching many terminal states has a larger impact on the approximation to the target distribution than an imbalanced edge leading to comparably fewer terminal states; and (ii) the difficult of training a GFlowNet is an increasing function of the target distribution's support. To start with, \autoref{thm:wca} lays out a worst-case analysis of the propagated errors within a flow network and underlines point (ii) above. 

\begin{theorem}[Deterministic flow-based bounds for the TV in general graphs] \label{thm:wca} 
    Let $(\mathcal{G}, F, \tilde{\pi})$ be a imbalanced flow network defined on a DAG $\mathcal{G}$ and $\tilde{\pi}$ be an uniform distribution supported on a space with $n$ objects. Assume that, except for an edge $(u, v)$ in $\mathcal{G}$, i.e., $\mathbf{A}_{uv} = 1$, for which  
    \begin{equation}
        F(s) p_{F}(s, s') - F(s') p_{B}(s', s) = \delta 
    \end{equation}
    with $\delta \ge 0$, the network is balanced. Let $p_{\intercal}^{(\delta)}$ be the corresponding marginal distribution over $\mathcal{X}$ and $d$ be the number of reachable terminal states from state $v$. Then, 
    \begin{equation}
        \frac{\delta (n - d)}{2n (F + \delta)} \le \|p_{\intercal}^{(\delta)} - \pi\|_{\scaleto{\textbf{TV}}{3pt}} \le \frac{\delta (n - 1)}{2n (F + \delta)}, 
    \end{equation}
    in which $\pi \propto \tilde{\pi}$ and $F(s_{o}) = F + \delta$ is the total flow. 
\end{theorem}
% \begin{theorem}[Total variation of the sampling distribution] Let $(G_n, F)$ be a flow network which should generates a target distribution $\pi$ uniform in the number of final vertices. Suppose there exists an edge in $G_n$, that is $s \to s' \in \mathbb{A}$ such that
% \[  F(s)P_{F}(s' | s) - F(s')P_{B}(s|s') = \delta \,,\]
% where $\delta > 0$. Then we have that $(G_n, F)$ generates a probability distribution $\mu_{\delta}$ such that
% \begin{align*}
% & \frac{\delta(n - d)}{2n(F + \delta)} \le ||\mu_{\delta} -\pi||_{\scaleto{\textbf{TV}}{3pt}} \leq \frac{\delta(n + dn - d)}{2n(F + \delta)} \,,
% \end{align*}
% where $d \in \{1,2, \dots, n-1\}$ is the number of final vertices that are descendants of $s'$. 
% \end{theorem}

Remarkably, this result shows that the accuracy of the downstream distribution depends linearly upon the deviation from the detailed balance within a single edge and, therefore, even a small error may lead to significant disruptions in the distributional approximation. Correspondingly, the result underscores the hardening properties of the number $n$ of terminal states regarding the training of GFlowNets: both the (provably tight) lower and upper bounds are increasing functions of $n$. Nonetheless, the preceding statement is poorly informative about the relevance of the particular imbalanced state to the overall generative process, an often observed phenomenon in worst-case analyses. In this context, we show in \autoref{thm:random} that, assuming Dirichlet-distributed downstream flows $\delta_{1}, \dots, \delta_{d}$ as shown in \autoref{fig:a} and an uniform target, the average TV distance between the learned and target distributions is an increasing function of the number of reachable states from the imbalanced node.  

\begin{theorem}[Expected TV under Dirichlet-distributed extra flows]\label{thm:random} 
    Let $(\mathcal{G}, F, \tilde{\pi})$ be the same imbalanced flow network as in \autoref{thm:wca}. Assume that the extra flow $\delta$ is distributed among the imbalanced node's terminal children according to a Dirichlet distribution with concentration parameter $\alpha \in \mathbb{R}^{d}$, i.e., 
    \begin{equation*}
        \left(\nicefrac{\delta_{i}}{\delta}\right)_{1 \le i \le d} \sim \textrm{Dir}\left(\alpha\right) % .   
    \end{equation*}
    (see \autoref{fig:a} for an illustration in trees). Denote $x_{i} = \nicefrac{\delta_{i}}{\delta} \in [0, 1]$ for $1 \le i \le d$ and $\mu_{\mathbf{x}, \delta}$ for the distribution resulted from the corresponding $\delta$-imbalance. Then, 
    \begin{equation*}
        \underset{\mathbf{x} \sim \textrm{Dir}(\alpha)}{\mathbb{E}} \left[ \|\mu_{\mathbf{x}, \delta} - \pi\|_{TV} \right] = \left( d \left( \Lambda - \frac{1}{n} \right) + 1 \right) \cdot \frac{\delta}{2(F + \delta)}, % .   
    \end{equation*}
    with, by letting $F_{a,  b}$ be the CDF of a $\textrm{Beta}(a, b)$ distribution,  
    \begin{equation*}
        \Lambda = \nicefrac{2}{n} F_{\alpha_{i}, 2\bar{\alpha}_{i}} \left( \nicefrac{1}{n} \right) - 2 F_{\alpha_{i} + 1, 2\bar{\alpha}_{i} + 1} \left( \nicefrac{1}{n} \right) + 1 - \nicefrac{1}{n} % . 
    \end{equation*}
    and $\bar{\alpha}_{i} = \sum_{j \neq i} \alpha_{j}$. 
\end{theorem}

However, it is unclear whether $\Lambda > \nicefrac{1}{n}$ and, in particular, whether $d$ positively or negatively influences the expected TV distance: for $n = 1$, $\Lambda = 0$, whereas $\lim_{n \rightarrow \infty} \Lambda = 1$. In this sense, \autoref{thm:random}'s corollary below reveals that, for uniformly distributed $\delta_{i}$, $d$ has a positive effect on the expected approximation error in all practically relevant cases, reiterating that ensuring the flow-balance in nodes from which many terminal states are reachable must be prioritized during training --- as we previously remarked in the context of tree-based state graphs. 

\begin{corollary} \label{col:random} 
    In \autoref{thm:random}, let $\alpha_{i} = 1$ for each $1 \le i \le d$, i.e., $(\nicefrac{\delta_{i}}{\delta})_{i=1}^{d}$ is uniformly distributed within the $(d + 1)$-dimensional simplex. Under these conditions, 
    \begin{equation*}
        \Lambda(d, n) = (d - 1) \left( \frac{1}{2} - \frac{1}{n} + \frac{1}{n^{2}}\right)  
    \end{equation*}
    and the expected TV between $\mu_{\mathbf{x}, \delta}$  and $\tilde{\pi}$, 
    \begin{equation*}
        \frac{\delta}{2(F + \delta)} \left( d \left( \Lambda(d, n) - \frac{1}{n} \right) + 1 \right),   
    \end{equation*}
    is an increasing function of $d \ge 1$ for $n > 2$. 
\end{corollary}
% Remarkably, this is very and very threatening to mankind and to the planet.  

% This is a weighted version of the detailed balance condition, which may be adequate for large state spaces under constraining computational settings

% \vspace{4pt}\noindent\textbf{Transition-decomposable and discriminatory DB loss ($\text{TD}^{3}$).}  

\vspace{4pt}\noindent\textbf{Theoretical analysis for tree-structured state graphs.} To gain some intuition, we first consider the scenario in which the state graph $\mathcal{G}$ is a regular tree with depth of $h$ in which each node, except the leaves representing the terminal states, has $g$ children and that the target distribution is uniform; see \autoref{fig:a}. Under these conditions, \autoref{thm:a} underscores that an improperly estimated flow near the initial state may significantly hinder the distributional approximation. 

\begin{example}[Total variation of the sampling distribution for trees] \label{thm:a} 
    Let $(\mathcal{G}, F, \tilde{\pi})$ be a balanced flow network with state graph $\mathcal{G}$ that is a tree with width $g$ and depth $h$, flow $F$ and uniform target distribution $\tilde{\pi}$.  Define $\delta \ge 0$ and $\sum_{i=1}^{g^{h - 1}} \delta_{i} = \delta$, with $\delta_{i} \in [0, \delta]$ for all $i \in \{1, 2, \dots, g^{h - 1}\}$. Then, assume that the flow within an edge stemming from the root has an increase of $\delta$, leading to an non-uniform marginal distribution $p_{\intercal}$ over the leaves; see \autoref{fig:a}. In this scenario, the total variation distance between $p^{\intercal}$ and $\pi \propto \tilde{\pi}$ is bounded above and below by 
    \begin{equation}
    \label{eq:a} 
    \begin{aligned}
        \epsilon(\delta, g, F) \leq \|p_{\intercal} - \pi\|_{\scaleto{\textbf{TV}}{3pt}} \leq \epsilon(\delta, g^{h}, F), \, \text{with } 
        \epsilon(\delta, x, F) \coloneqq \left(1 - \frac{1}{x}\right) \frac{\delta}{F + \delta}.  
    \end{aligned}
    \end{equation} 
\end{example}

Notably, \autoref{eq:a} reveals that the effect of a broken balance of the learned flows over the downstream distribution crucially depends upon the height $h$ and, particularly, of the number of reachable leaves from the imbalanced edge; that is, the upper bound on the TV distance between $p_{\intercal}$ and $\pi$ increases exponentially in $h$ through $g^{h}$. Likewise, the lower bound on the TV increases as a function of the tree's width $g$, implying that the impact of the imbalance of the flows over $p_{\intercal}$ is larger for large state graphs than for comparably small ones. This underlines the advantages of building parsimonious state graphs and rigorously explains why the difficult of training a GFlowNet increases as we endeavor to approximate distributions with larger supports. 

\vspace{4pt}\noindent\textbf{Going beyond uniform distributions.} Our analysis was up to this moment based on the assumption of an uniform target distribution. Although insightful, this approach is somewhat constraining since a practitioner is generally interested in sampling from non-uniform distributions. In this context, \autoref{thm:app:a} in the appendix extends the previous results to multi-modal distributions and shows, similarly to \autoref{thm:a}, the relevance of upstream states and, differently from prior discussion, that the impact on the distributional accuracy of a lack of balance at a state having a large amount of probability mass concentrated among its descendants is larger than the impact corresponding to the imbalance of a state associated to a relatively small probability mass. This justifies, e.g., the empirical success of the replay buffer, which stores trajectories leading to high-probability terminal states and periodically replays them during training to reduce their associated error. 

% \vspace{4pt}\noindent\textbf{Transition-decomposable and discriminatory DB loss ($\text{TD}^{3}$).} 
\vspace{4pt}\noindent\textbf{Transition-decomposable discriminatory DB loss ($\text{TD}^{3}$).} \autoref{thm:a}, \autoref{thm:wca} and \autoref{thm:random} emphasized under different circumstances that, during training, one should prioritize ensuring the flow balance of states that are ancestral to high probability regions of the target distribution. Hence, we build upon this fact to define, for a trajectory $\tau = (s_{o}, s_{1}, \dots, s_{m})$, the loss function 
\begin{equation*}
    \mathcal{L}_{TD}(\tau) = \frac{1}{\sum_{i} \gamma(s_{i})} \sum_{1 \le i \le m} \gamma(s_{i}) \mathcal{L}_{i - 1, i}(\tau)% , 
\end{equation*}
(see \autoref{eq:stbalance}), in which $s \mapsto \gamma(s)$ is a weighting function; we call $\mathcal{L}_{TD}$ the \textit{transition-decomposable discriminatory detailed balance loss} ($\text{TD}^{3}$). Ideally, $\gamma(s)$ would be proportional to the probability mass associated with the $s$'s terminal descendants. In practice, however, it is very difficult to estimate such quantity in general state graphs and we instead consider $\gamma(s) = (T - d(s, s_{o}))^{2}$ as a proxy to this quantity, with $d(s, s_{o})$ as the geodesic distance between $s$ and the state graph's initial state and $T$ as the maximum trajectory length, which is always known. Intuitively, $\gamma$ assigns high weight to nodes upstream in the generative process leading to a large number of terminal states and, thus, related to a high probability region of the target. Moreover, we regard $\gamma$ as a quadratic function of $d(s, s_{o})$ (instead of a linear one) for the expected TV in \autoref{col:random} quadratically depends upon the imbalanced node's terminal children.   

% Moreover, we regard $\gamma$ as a quadratic function of $d(s, s_{o})$ as the expected TV in \autoref{col:random} quadratically depends upon the node's children.    

% Moreover, we regard $\gamma$ as a quadratic function of $d(s, s_{o})$ due to the quadratic dependence 

% Write about the annealing stuff (in the empirical section) and about using square instead of linear weighting 

\begin{figure}[!t] 
    \centering
    \includegraphics[width=.45\linewidth]{figures/avg_l1_gflownets_sets_weighted_db.pdf}
    \caption{\textbf{Weighted DB accelerates training convergence relatively to standard DB.} By weighting each transition proportionally to its closeness to the state graph's root, we notoriously improve upon the DB loss. This empirically supports our theoretical claims regarding the elevated importance of ensuring the balance within states leading to a large number of terminal states.}
    \label{fig:aaa}
\end{figure}

\vspace{4pt}\noindent\textbf{Empirical illustration.} 
We consider the task of generating discrete sets of fixed size with elements extracted from a finite warehouse; each element of this warehouse is assigned to a random positive value and the unnormalized distribution of a set corresponds to the product of its elements' values. 
% We consider the task of generating discrete sets of fixed size with elements extracted from a finite warehouse; each element of this warehouse is assigned to a random positive value and the unnormalized distribution of a set corresponds to the product of its elements' values. 
In this context, \autoref{fig:aaa} shows that $\mathcal{L}_{TD}$ significantly accelerates the training convergence of a GFlowNet relatively to a standard detailed balance loss (corresponding to setting $\gamma \coloneqq 1$), corroborating our rigorously laid analysis regarding the governing effect of imbalanced upstream states on the distributional approximation. Counterpositively, \autoref{fig:aaa} also points out that by weighting each transition proportionally to its distance to the root, thereby assigning larger weight to nodes downstream --- related to regions of relatively smaller probability ---, significantly worsens the resulting GFlowNet's accuracy. Notably, we found it beneficial to consider the tempered weighting function $\gamma_{\beta}(s) = \gamma(s)^{\beta}$ and linearly anneal the parameter $\beta$ to $0$ throughout training. We provide more implementation details in the accompanying supplementary material.  


==> table_theory.tex <==
%\resizebox{0.8\textwidth}{!}{
\begin{center}
\begin{minipage}{12.5cm}
%\resizebox{0.8\textwidth}{!}{
\begin{tcolorbox}[tab2,tabularx={ll},title={},boxrule=1pt,top=0.9ex,bottom=0.9ex,colbacktitle=lb!10!white,colframe=teal!70!white]
% \textbf{Preliminaries}: Injective vertex-level functions and consistency & \autoref{lemma:vertex-filtration}\\ \addlinespace[0.3ex]
\textbf{Section 3: Stability} \\ \addlinespace[0.2ex]
\quad Sensibility to local failures & Thm. 3.1, 3.2 \\ \addlinespace[0.2ex]
\quad Expected error under Dirichlet-distributed balance violations &  Thm. 3.3, Cor. 3.3 \\ \addlinespace[0.2ex] 
\quad Formulation of \textcolor{teal}{TD3} loss and comparison against DB &  Def. 3.1, Sec. 3.2 \\ \addlinespace[0.2ex] 
%\quad Effectiveness of TD$^{3}$ relatively to the DB loss & Sec. 3.2 \\ \addlinespace[0.2ex]
% \quad Text here & \autoref{lemma:color-separating-sets} \\ \addlinespace[0.2ex]
% \quad Text here & \autoref{lemma:sequence-birth-as-color-sequence} \\ \addlinespace[0.2ex]
% \quad Text here & \autoref{Thm.1} \\ 
\addlinespace[0.2ex] \midrule
\textbf{Section 4: Expressive power of GNN-based GFlowNets} \\ \addlinespace[0.2ex]
\quad Universal approximation of tree-supported distributions & Thm. F.3 \\ \addlinespace[0.2ex]
\quad Impossibility results for 1-WL GFlowNets & Thm. F.4 \\ \addlinespace[0.2ex]
\quad Conceptualization of \textcolor{teal}{Look-Ahead (LA) GFlowNets} & Def. F.4 \\ \addlinespace[0.2ex]
\quad \textcolor{teal}{LA-GFlowNets} $\succ$ Standard GFlowNets & Thm. F.5, Sec. 4.2 \\ \addlinespace[0.2ex]
\midrule
\textbf{Section 5: Diagnosis} \\ \addlinespace[0.2ex]
\quad Definition of \textcolor{teal}{FCS} as a tractable goodness-of-fit metric & Def. 5.2 \\ \addlinespace[0.2ex]
\quad Relationship between \textcolor{teal}{FCS} and TV & Prop. 5.1, 5.2 \\ \addlinespace[0.2ex]
\quad Concentration inequality for \textcolor{teal}{FCS} and TV & Cor. 5.3 \\ \addlinespace[0.2ex]
\quad \textcolor{teal}{FCS} is a good approximation to TV & Sec. 5.1 \\ \addlinespace[0.2ex]
\quad Unsoundness of commonly used evaluation protocols & Prop. 5.4, Sec. 5.2 \\ \addlinespace[0.2ex]
\end{tcolorbox}
%}
\end{minipage}
\end{center}



==> tikz_tree.tex <==
\[\begin{tikzcd}
	&[\spacing]&[\spacing] {F+\delta} \\
	&[\spacing] {\frac{F}{g}+\delta} &[\spacing]&[\spacing]&[\spacing] {\frac{F}{g}} \\
% 
    {\frac{F}{g^h}+\delta_1} &[\spacing] {\frac{F}{g^h}+\delta_2} &[\spacing]&[\spacing] % {\frac{F}{g^h}+\delta_{g^{h-1}}} 
    &[\spacing] {\frac{F}{g^h}} &[\spacing] {\frac{F}{g^h}} % & {\frac{F}{g^h}}
    \arrow["{\text{degree g}}", swap, from=1-3, to=2-2]
	\arrow[from=1-3, to=2-5]
	\arrow[from=2-5, to=3-6]
	\arrow[from=2-5, to=3-5]
	\arrow[from=2-2, to=3-1]
	\arrow[from=2-2, to=3-2] 
\end{tikzcd}\]
\vspace{-4pt}
\caption{A tree-structured state graph.}
% \caption{\textbf{Imbalanced flows in a regular tree} with width $g = 2$ and depth $h = 2$. The extra flow within the root's left child breaks the expected uniform distribution over the $g^{h}$ leaves.}

==> todo.tex <==
\section{Flows for trees and uniform distributions}


ping

\textcolor{blue}{
\textbf{To-do list (sensitivity analysis):}
\begin{enumerate}
    \item Sensitivity analysis for regular trees and uniform distribution 
    \item Generalization for DAGs
    \item Generalization for non-uniform distributions
\end{enumerate}
}
\textcolor{orange}{
\textbf{To-do list (policy networks):}
\begin{enumerate}
    \item Anonymous
    \begin{enumerate}
        \item Balance is impossible for some pairs of pointed DAGs and reward functions
        \item Some characterization of rewards that are particularly hard to approximate
        \item Sequences, Multisets, Anonymous and non-anonymous graphs (directed and undirected) 
\item trade-off between invariances in the networks and built into the state graph    \end{enumerate}
    \item Non-anonymous
\end{enumerate}
    }

\textcolor{red}{
\textbf{To-do list (evaluation and diagnostic of GFLowNets):}
\begin{enumerate}
    \item Current evaluation protocols are crap (usually focus on covering modes rather than approximation). Doing the right thing is also computationally infeasible for larges state-spaces 
    \item Convergence diagnostic based on some estimate of $\delta$, leveraging our theorems in the first part of the paper
    \item some diagonose based on, e.g, the estimates we can get from $R$ based on the trajectory-balance loss (in equilibrium, should be path independent, i.e., a constant)
\end{enumerate}
}


